Refactoring Practices in the Context of Modern Code Review: An Industrial Case Study at Xerox

Modern code review is a common and essential practice employed in both industrial and open-source projects to improve software quality, share knowledge, and ensure conformance with coding standards. During code review, developers may inspect and discuss various changes including refactoring activities before merging code changes in the codebase. To date, code review has been extensively studied to explore its general challenges, best practices and outcomes, and socio-technical aspects. However, little is known about how refactoring activities are being reviewed, perceived, and practiced. This study aims to reveal insights into how reviewers develop a decision about accepting or rejecting a submitted refactoring request, and what makes such review challenging. We present an industrial case study with 24 professional developers at Xerox. Particularly, we study the motivations, documentation practices, challenges, verification, and implications of refactoring activities during code review. Our study delivers several important findings. Our results report the lack of a proper procedure to follow by developers when documenting their refactorings for review. Our survey with reviewers has also revealed several difficulties related to understanding the refactoring intent and implications on the functional and non-functional aspects of the software. In light of our findings, we recommended a procedure to properly document refactoring activities, as part of our survey feedback.

==> Tables/CodeReview.tex <==
\begin{table*}
  \centering
	 \caption{Related Work in Code Review}
	 \label{Table:Survey CR}
%\begin{sideways}
\begin{adjustbox}{width=1.0\textwidth,center}
%\begin{adjustbox}{width=\textheight,totalheight=\textwidth,keepaspectratio}
\begin{tabular}{lcllllll}\hline
\toprule
\bfseries Study & \bfseries Year  &  \bfseries Research Type & \bfseries Purpose & \bfseries Evaluation technique  & \bfseries Refactoring? \\
\midrule
Tao et al. \cite{tao2012software} & 2012 & Industrial Survey & Understand code changes during development process & Survey 180 engineers \& managers & No \\ \hline
Bacchelli \& Bird  \cite{bacchelli2013expectations} & 2013 & Industrial Survey & Understand the motivations, challenges, and outcomes of tool-based CR  & Survey 165 managers \& 873 programmers & No \\
& & & & Interview 17 developers \\ \hline
McIntosh et al. \cite{mcintosh2014impact,mcintosh2016empirical} & 2014 & Empirical \& Case Study & Study the impact of CR coverage \& participation on quality & Case study of 3 OSS & No \\ \hline
Ge et al. \cite{ge2014towards,ge2017refactoring} & 2014,2017 & Tool-based code review & Detect refactoring from non-refactoring changes & Case study of 2 OSS & Yes \\ 
& & & & Formative study of 35 developers \\ \hline 
Alves et al. \cite{alves2014refdistiller,alves2017refactoring} & 2014,2018 & Tool-based code review & Inspect manual refactoring edits & Tool assessment using 3 OSS &  Yes\\
& & & & User study with 15 developers \\ \hline
Morales et al. \cite{morales2015code} & 2015 & Empirical study & Understand the impact of code review on quality & Case study of 3 OSS &  Yes \\ \hline
Barnett et al.\cite{barnett2015helping} & 2015 & Industrial User Study & Introduce automatic decomposition of CR & Interview 20 developers & No \\ \hline
Tao \& Kim \cite{tao2015partitioning} & 2015 & Empirical \& User Study & Partitioning composite code changes for CR & User study of 18 CS students & No \\ \hline
Zhang et al. \cite{zhang2015interactive} & 2015 & User Study & Present interactive CR for systematic changes & User study (1) of 6 engineers & No  \\ 
& & & & User study (2) of 12 engineers \\ \hline
MacLeod et al.  \cite{macleod2017code} & 2017 & Industrial Survey & Understand challenges \& best practices of CR & Interview 18 developers & No \\ 
& & & & Survey 911 developers \\ \hline
Sadowski et al. \cite{sadowski2018modern} & 2018 & Industrial Case Study \& Survey & Investigate MCR in industry & Intrervew 12 developers &  No \\ 
& & & & Survey 44 Engineers & \\ \hline
Coelho et al. \cite{coelho2019refactoring} & 2019 & Systematic mapping study & Present refactoring solutions to MCR & N/A &  Yes \\ \hline
Pascarella et al. & 2019 & Empirical study & Study the effect of code review on code smells & Analysis of 7 OSS & Yes  \\ 

\bottomrule
\end{tabular}
\end{adjustbox}
%\end{sideways}
\end{table*}

